Interpreting search result rankings through intent modeling

Given the recent interest in arguably accurate yet non-interpretable neural models, even with textual features, for document ranking we try to answer questions relating to how to interpret rankings. In this paper we take first steps towards a framework for the interpretability of retrieval models with the aim of answering 3 main questions "What is the intent of the query according to the ranker?", "Why is a document ranked higher than another for the query?" and "Why is a document relevant to the query?" Our framework is predicated on the assumption that text based retrieval model behavior can be estimated using query expansions in conjunction with a simpler retrieval model irrespective of the underlying ranker. We conducted experiments with the Clueweb test collection. We show how our approach performs for both simpler models with a closed form notation (which allows us to measure the accuracy of the interpretation) and neural ranking models. Our results indicate that we can indeed interpret more complex models with reasonable accuracy under certain simplifying assumptions. In a case study we also show our framework can be employed to interpret the results of the DRMM neural retrieval model in various scenarios.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

Version 1.36    Bug fixes
		Moved PACMPL to acmlarge format
		New journal: PACMHCI
		Added the possibility to adjust number of author
		boxes per row in conference formats
		
Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
		Added processing of one-compoment ccsdesc nodes
		Bug fixes.
		Made the height a multiple of \baselineskip + \topskip
		Added cleveref
		We no longer print street address in SIGs

Version 1.41    Rearranged bib files
		Added new badges

Version 1.42    Deleted ACM badges
		Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
		Empty DOI and ISBN suppress printing DOI or ISBN lines
		Separated theorem code into acmthm.sty, loaded by default.
		Article number can be set for proceedings.
		New commands: \acmBooktile, \editor.
		Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
		from Overleaf

Version 1.46    Bug fixes for bibliography:  label width is now calculated
		correctly.
		All PACM now use screen option.  This requires etoolbox.
		Added subtitle to ACM reference format.
		Now acmart is compatible with fontspec.
		\thanks is now obsolete.  The addresses are automatically
		added to the journal version;  this can be overriden with
		\authorsaddresses command.
		Deleted the rule at the end of frontmatter for all formats.
		Deleted new line before doi in the reference format.
		Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal:  THRI

Version 1.48    Bug fixes
		Review mode now switches on folios

==> old_intro.tex <==
\section{Introduction}
\label{sec:intro}

% Figure~\subref{fig:list} shows an   Figure~\subref{fig:single} demonstrates 

% \begin{figure}[t!]
%     \centering
%     \begin{subfigure}[t]{0.3\textwidth}
%         \centering\captionsetup{width=.8\linewidth}%
%         \includegraphics[width=0.8\textwidth]{figs/doc_compare.png}
%         \label{fig:list}
%         \caption{ The intent terms identified are \textit{america}, \textit{defeat} and \textit{war}. The overall size of the bar below each document title indicates the relevance score as estimated by the local explanation model. Immediately we can see how relevance varies across the documents. Even though the second document contains all terms and has a higher score for the query terms, the reason why it is ranked second is due to the term \textit{defeat}.}
%     \end{subfigure}%
%     ~ 
%     \begin{subfigure}[t]{0.3\textwidth}
%         \centering\captionsetup{width=.5\linewidth}%
%         \includegraphics[width=0.97\textwidth]{figs/single_doc.png}
%         \caption{How to explain the relevance score of a single document. For this query, our explanation indicates that the complex ranker relies heavily on frequency but for the query terms proximity is also important.}
%         \label{fig:single}
%     \end{subfigure}
%     \caption{Anecdotal visualization of explanations based on uncovered intent terms for the query \texttt{afghan flag} and a complex ranker \bbranker like a neural network. }
%     \label{fig:viz_afghan}
% \end{figure}



% Why is interpretability important ?
\mpara{Why Interpretability ?} In the context of data-driven models, interpretability can be defined as ``\textit{the ability to explain or to present in understandable terms to a human}''~\cite{doshi2017towards}. For the most part, machine learnt models are used as black boxes which output a prediction, score or ranking without understanding partially or even completely how different features influence the output. In such cases when an algorithm prioritizes information to predict, classify or rank; algorithmic transparency becomes an important feature to keep tabs on restricting discrimination and enhancing explainability-based trust in the system. Recently, in the machine learning (ML) and NLP communities there has been growing interest in the interpretability of ML models~\cite{binder2016layer,nlp2015visualizing,lei2016rationalizing} but there has been limited work on interpreting retrieval models considered central in IR.  

\mpara{Learning complex rankings.} When using machine learning models to rank results, the training data (clicks, human annotations) informs how signals/features should be combined. Various models have been employed, ranging from linear regression and decision trees to deep neural networks~\cite{mitra2017neuralCIKM,dehghani2017neural,hui2017position,desm16} more recently. On a more abstract level, by learning how to combine features to best rank documents, the machine learned model is indirectly encoding the query intent. Documents are then ordered by relevance, i.e. how well to do they match the underlying query intent.

In this paper we focus on interpreting complex ad-hoc ranking models like deep neural nets that automatically learn representations and features. These models are increasingly popular due to improved performance but their decisions are hard to interpret.
%learned from existing training data and more specifically we would want to understand complex models that deal with text features. 

% Given the recent interest in arguably accurate yet non-interpretable neural models, even with textual features such as DRMM~\cite{guo2016deep} and DSSM~\cite{mitra2017neural}, for document ranking we try to answer questions relating to how to interpret rankings. 
% Such models are not only used in document search applications but also in the candidate ranking phase for applications like conversational search and open domain question answering. 

%We believe that the groundwork laid in this paper will help us further tackle models that use a variety of features from  both the content and external sources like user behavior patterns, authority measures, knowledge bases etc. 

% Departing slightly from the data centric view, we focus on the mechanics behind the construction of a ranked list. 

\mpara{Interpreting intents in rankings. } We first ponder on what interpreting a rankings really means. Are we interested in explaining why a document was relevant or ranked above another ? Although that is certainly interesting, what we are really interested in is if a model is performing in accordance with the \emph{information need} of the user who issues the query -- a central concept in IR. In other words, what is the actual query intent as understood by the trained model. 

% Interpreting the information need of a user from a user specified query is key to IR.
% However the key difference in interpreting a ranker is that we are trying to explain what the model has actually understood as the intent which in turn caused the resulting rank output. In essence we are trying to interpret the model understanding of the information need of the user.

% Chief among these are neural rankers that have gained popularity recently with state of the art performance by automatically learning representations and scoring functions from training data. 

There are two key benefits to uncovering the learned intent. First, users can immediately identify biases induced by varied training data. For example, consider the query \textit{afghan flag} and two different rankers:

\textbf{Ranker 1 Top Doc:} \texttt{American invasion leads to burning of afghan flags ...}

\textbf{Ranker 2 Top Doc:} \texttt{Americans share experience of visit to Afghanistan ...}

Both rankers seemingly prefer documents about Americans in Afghanistan but why they choose different top documents is unclear. However if we present the user with terms that encode the intent then this becomes easier to discern. The intent of \textbf{Ranker 1} is \{\texttt{war, america, conflict, soldier, defeat}\} and that of \textbf{Ranker 2} \{\texttt{pole, mast, hoist, tourist, nation, anthem}\}. Ranker 1 seems to be trained from a time period where the war in Afghanistan was more relevant whereas Ranker 2 does not seem to be biased towards this event.

The second benefit is being able to help identify overfitting or under-performance. If spurious patterns like copyright messages are identified as part of the intent, developers can quickly rectify the data and improve the model. 

While terms are easy to understand as explanations, it may not be enough to accurately answer two important questions: Why is A relevant? Why is A ranked above B? Hence we also need a model that can easily explain how a document is relevant to the query using the intent terms. 
\todo{A line about how we model intents and what is our explanation. Details of the problem like maximization of pref. pairs can be left out}

\mpara{Post-hoc interpretability.} Approaches in interpretability can be broadly classified into models that are \emph{interpretable by design} and approaches that explain an already built model or \emph{post-hoc interpretability}. Models that are interpretable by design use training procedures and features that are themselves interpretable like decision trees, falling rule lists etc. However, they do not possess the modeling capacity, and hence are not as accurate as, of modern and more recent complex models. We therefore, focus on the post-hoc interpretability of learnt rankers that enables us to tackle a multitude of text based retrieval models irrespective of the underlying learning algorithm or training data.

\mpara{Our Approach.} A ranking task is different other supervised tasks in that it can viewed as an aggregation of multiple decisions -- either ordering multiple relevant documents or resolving pairwise preferences. This also makes applicability of previous works on simpler supervised tasks difficult.
% We tackle this challenge by explicitly exploiting the preference information between pairs of documents to ascertain relevant intents. 
We approach the problem of post-hoc interpretation of a black-box ranking model for a query by learning a simple ranking model, with an expanded query, that approximates the original ranking. In doing so, we 
argue that the expanded query forms the intent or explanation of the query \emph{as perceived by the black-box ranker}. In coming up with the explanation or the intent we hypothesize that an expanded query, using a simpler and interpretable model, is an accurate interpretation of the black-box model if it produces a similar ranking to the ranking of the black-box model. Towards this we exploit the pairwise preferences between documents in the original ranking to extract relevant terms to be considered for expansion by postulating a combinatorial optimization problem called the \problem. We further reduce the effect of false positive terms by novel document perturbation techniques.

We conducted experiments with the Clueweb test collection. We show how our approach performs for both simpler models with a closed form notation (which allows us to measure the accuracy of the interpretation) and neural ranking models. Our results indicate that we can indeed interpret more complex models with reasonable accuracy under certain simplifying assumptions. In a case study we also show our framework can be employed to interpret the results of the DRMM neural retrieval model in various scenarios.
 
% Our approach to generating explanations of learned intent takes advantage of document preference pairs that can be extracted from a ranking. The set of terms that preserves the maximum number of preference pairs according to an appropriate scoring function forms the explanation of the underlying intent. 

% For both questions, indicating the mere presence or absence of intent terms in a document can help users already. However this is not useful in cases where the difference in relevance is more fine grained. When A and B both contain the same explanation terms there is a need for an enriched explanation. Frequency, position and proximity of term occurrence are vital to rankers and should be factored into the explanation. Therefore the key to answering the aforementioned questions is to not only identify the intent terms but also estimate how the ranker scores terms. This will allow for explanations as shown in Figure~\ref{fig:viz_afghan} which can significantly improve our understanding of complex ranking models.  





% \begin{figure}[ht]
% 	\includegraphics[width=0.35\textwidth]{figs/shoes.pdf}
%     \caption{Top 3 product titles for two different rankers for the query \textit{dress shoes}}.
%     \label{fig:shoes}
% \end{figure}




==> setup-old.tex <==
% \newpage

\section{Experimental Setup}

In this section we detail the experimental setup to test our hypothesis of using terms that encode intent as expansions along with a simple ranker to approximate \bbranker(q). Note that we restrict ourselves to bag-of-words based \bbranker. We leave blackboxes that take sequences, term proximity and position into account for future work. 

%In this section we detail the experimental setup for the both, strongly agnostic and weakly agnostic scenarios. First we describe the commonalities and then describe key differences and approach variants considered. 

\textbf{Data:} For all experiments we use the web track Clueweb09 TREC test collection meant for adhoc retrieval. We use the category B subset which contains 50 million web pages. Lucene was used to index the collection. For text preprocessing, Lucene's English Analyzer was used. We use all 300 queries for the strongly agnostic case and the first 200 queries for the weakly agnostic case. For each query in the test collection we retrieve the top 1000 documents ranked by a statistical language model with Dirichlet smoothing($\mu=2000$). We remove spam documents using the Waterloo spam list~\cite{cormack2011efficient}. 

\textbf{Sampling Preference Pairs/Features:} Optimizing for all preference pairs is prohibitively expensive for most queries in the web track. In our experiments we study the effect of 4 different preference pair sampling techniques on the quality of the explanation produced. 

\begin{enumerate}
\item \random: Randomly select preference pairs from the target ranking.
\item \rankbiased: Sample preference pairs from the target ranking that are weighted by rank. Each pair is weighted by $1/rank(d_i) + 1/rank(d_j)$.
\item \topkrankrandom: Construct preference pairs based on a combination of rank and random sampling. In this method, for a preference pair $(d_i > d_j)$, $d_i$ is first rank bias sampled and then $d_j$ is randomly sampled. In addition, we consider all pairs from the top-k results to explain.
\item \topkrandom:  We consider all pairs from the top-k results to explain and a fixed number of randomly sampled pairs.
\end{enumerate}
 We contrast these against \topk (no sampling; consider only all pairs from the top-k results to explain). 
Furthermore, we experiment with varying the number of samples for each technique and observe its effect on the metrics mentioned below.

\textbf{Metrics:} We use 4 metrics to measure the efficacy of our approach. To measure the utility of the explanation we use two measures of fidelity based on Kendall's $\tau$ which is used to measure rank correlation between two lists. 

\textit{Local fidelity} is $\tau$@k between \bbranker's top-k documents ranking and the corresponding ranking by \explainer for ($q \cup T_q$). \textit{Global fidelity} is computed between the rankings produced by \explainer($q \cup T_q$) and \bbranker(q) for all documents returned from the index (after spam filtering) for the given query.

%Let ${\mathcal{U}_{q}}^{10}$ refer to the set of all concordant pairs from top 10 documents for a given $q$ and $\mathcal{R}$. Let ${{U}_{q}}^{10}$ refer to the pairs in the top 10 that can be explained with $E_q$. Then local fidelity $f_q@10 = \frac{|{{U}_{q}}^{10} \cap \mathcal{{U}_{q}}^{10}|}{ | \mathcal{{U}_{q}}^{10} |}$. Similarly, if we assume $\mathcal{U}_{q}$ is the set of all/sampled pairs for a given $q$ and $\mathcal{R}$, then global fidelity is $F_q = \frac{|{U}_{q} \cap \mathcal{{U}_{q}}|}{ | \mathcal{{U}_{q}} |}$.

%\todo{We might need to clarify $E_q, \mathcal{G}_{q} ,C_q ,U_q , \mathcal{U}_q$.Or introduce this before in the notations. This is different from what we had before.}

Explanations with high fidelity however may not be right for the right reasons. False positive terms cause overfitting to the document pairs selected for optimization. 
We measure the \textit{accuracy} of the explanation by computing the fraction of $T_q$ terms that overlap with the set of ground truth terms $\mathcal{G}_q$. 
To ensure that terms in $\mathcal{G}_q$ are present after the candidate selection procedure, we also report \textit{recall} values. Recall is computed as the fraction of candidate terms (from which $T_q$ is selected) that overlap with $\mathcal{G}_q$. 
%Note that if we consider all terms in the ranked list $\mathcal{R}(q)$, then recall is $1.0$ for \bbranker used in our experiments. 

%As mentioned earlier, considering all terms in the top 1000 documents can be expensive. Hence we devise an initial candidate term selection phase and measure the recall. 

We select the top-10 documents to explain for a given $q$ and \bbranker and set max $|T_q|$ to 10 in all our experiments. Note that in our experiments we are more interested in showing that our approach can be applied to a variety of retrieval models rather than the same retrieval model across multiple test collections. We believe our results are tied more to the models than the documents on which they are used. 
%Hence the reason we consciously chose to experiment using a single test collection.

%To measure the local fidelity of the explanations we use two separate metrics. First we use spearman's coefficient as a measure of rank correlation. If $T_q$ is an accurate explanation then the correlation between the top k produced by $\mathcal{R}$ using q and $R$ using $T_q$ should be highly correlated. However this may not still accurately capture how $\mathcal{R}$ estimates the relevance of a document for a given query. To further test the fidelity of the explanation we measure the recall of $T_q$ given the query expansions used by $\mathcal{R}$ which is a retrieval model utilizing query expansions through pseudo relevance feedback. 

%\subsubsection{Objective - Rank Correlation}

%\subsubsection{True fidelity check with query expansion based RMs}

%Let $\mathcal{R}$ be a retrieval model that expands $q$ with a set of terms $\mathcal{T}_{q}$ before using $R$ to rank the retrieved documents. $\mathcal{T}_{q}$ can be determined in several ways. We experiment with the following methods: pseudo relevance feedback, word embeddings and topic models.  

%We compare our results against LIME which is a framework for explaining the decisions of any classifier. We modify LIME to suit the ranking scenario by:


\textbf{Blackbox ranker \bbranker selection rationale:} We select 4 variants of blackbox rankers that internally utilize query expansions to explicitly encode intent and language models to score documents. The main reason behind choosing simple \bbranker's is the difficulty in identifying the correct intent terms for standard learning to rank models trained on judgements or click through. Without proper $\mathcal{G_q}$ we cannot effectively measure the accuracy of the explanation. This query expansion mechanism of the blackbox allows us to exactly identify the ground truth explanation terms $\mathcal{G}_q$. The closed-form notation of the scoring function (language model) $\mathcal{R}$ allows us to be certain that only term frequency and document length based statistics were used. Note that the input to \bbranker is still $q$ but it internally uses $\mathcal{G}_q$ and $\mathcal{R}$ to judge relevance.

This setup reflects previous interpretability works in the ML community. If an explanation model can correctly locally interpret a simple well understood model disguised as a blackbox then it is assumed to be powerful enough to locally interpret truly complex models. An example of such a setup for classification models can be found in~\cite{ribeiro2016model}.

%We use query expansions generated from different sources to expand a given query and then, using a language model, re-rank the documents. 

\textbf{Blackboxes selected:} We first devised 3 different non-neural black box rankers. For all we use a language model with Jelinik-Mercer smoothing with $alpha=0.4$ as $\mathcal{R}$. We specifically chose this setting to make it different from \explainer (described later).

\begin{equation}
P_{\mathcal{R}}(d|q) = \prod_{q_i \in q} \alpha P(q_i|d) + (1-\alpha)P(q_i|\cD)
\end{equation}

For the expansions we used two distinct approaches: pseudo-relevance feedback and word embeddings. We chose exactly 10 expansion terms per query for each of the following blackboxes: 

%This allows us to exactly identify the explanation terms $\mathcal{G}_q$. By using a language model to score documents we are fully aware of the scoring procedure for each document.

\begin{enumerate}
\item \textsc{RM3-10}: Using the RM3~\cite{lavrenko2017relevance} algorithm, we determined a set of relevant expansion terms from the top 10 documents for a given query. We then re-ranked the results using the aforementioned language model.

\item \textsc{RM3-20}: Similar to \textit{RM3-10}, except that the depth of the pseudo-relevant set is increased to 20.

\item \textsc{EMB}: Instead of using pseudo-relevant documents to find expansion terms, an external collection is used for the expansions. We use glove embeddings (300 dimensions) trained on a 2016 english Wikipedia dump to find semantically related terms. We first average the embeddings of the words in the query to create a query vector. Next we search the embedding space for the 10 nearest terms that also occur in the top 10 documents. 

\end{enumerate}

Our last \bbranker is a variant of the \textsc{DESM} neural retrieval model~\cite{mitra2016dual}. DESM models the relevance score of $d$ given $q$ as a parametrized sum between the syntactic relevance and semantic similarity between a learned query vector representation and the document vector representation.

\begin{equation}
P(d|q) = \gamma \prod_{q_i \in q} P_{MLE}(q_i|d) + (1-\gamma) P_{sem}(q|d)
\end{equation}

where $P_{sem}(q|d)$ is the cosine similarity between the query and the document representations. DESM's $P_{sem}$ component violates our basic assumption that presence of a relevant term monotonically increases $P(d|q)$. Depending on how the vectors are computed, $P_{sem}$ can vary drastically. The frequency, position and order in which terms occur (including non-relevant terms) can influence how semantically related a document is to a query. The parameter $\gamma$ allows us to trade off the semantic match systematically. When $\gamma$ is 1.0, all our assumptions hold true but as it decreases the assumptions don't always hold. 

We select terms closest to the query vector that are also present in the top 50 documents of the initial result list as $\mathcal{G}_q$. To compute the vectors we employ the same glove embeddings from \textsc{EMB}. The query vector is computed as an IDF weighted average of terms in the expanded query that have embeddings. We ignore queries where none of the terms have existing embeddings. For document embeddings we use a TF-IDF weighted average of terms in the document (while ignoring out of vocabulary terms). We set $\gamma$ to 0.9 in our experiments to limit the influence of the hard to interpret $P_{sem}$. 



%Here \bbranker is essentially a model that expands a query and scores documents using a language model that favors the collection probability $P(q_i|\cD)$. The expansion terms form the ground truth set $\mathcal{G}_q$ against which accuracy and recall are measured. 



% need a better line to justify why we chose this LM
\textbf{Explanation engine}: While accuracy is measured against $\mathcal{G}_q$, fidelity however is sensitive to the choice of \explainer used to estimate $\mathcal{R}$. For the explanation engine we fix \explainer as a language model estimated using MLE with additive smoothing, i.e., $P(q_i|d) = \frac{count(q_i, d)}{|d|}$. We had to be careful in choosing a language model that is sufficiently different from the ranking function in $\mathcal{R}$ since we are only concerned with bag of words based models. 

We select the top 1000 terms as candidates for the strongly agnostic scenario. For the weakly agnostic case we use perturbation to filter out potential false positives. First we select the top 500 terms after reductive perturbation on a sample of documents. We further halve the candidate set using additive perturbation on the top-k documents-to-explain resulting in a final candidate set of 250 terms. Table~\ref{tab:recall} shows the recall of the candidate set before and after perturbation. 

%The preference matrix formed had 250 rows at most when compared to the strongly agnostic case that has a 1000. We only use the documents from the sampled preference pairs for reductive perturbation.  In the additive perturbation stage we only perturb the the top-k documents that need to be explained.



%The top 1000 terms from the candidate generation technique described in Section~\ref{sec:cand-selection} are used as candidates. In this setting we do not remove false positives by perturbation.

%\subsection{Weakly Agnostic}

%\textbf{Blackboxes (\bbranker):} We devised 4 different 

%Like with the strongly agnostic case, 10 expansion terms are selected in order to measure accuracy. 

%These terms ($\mathcal{G}_q$) are then used by the DESM \bbranker to produce the target ranking $\mathcal{R}(q)$.



%We consider 4 variants by altering $\gamma$. Note that by setting $\gamma$ to 1.0, we ignore $P_{sem}$. In this case the ranking only depends on the terms in $\mathcal{G}_q$. Our approach for weakly agnostic scenarios includes a step to perturb documents in order to reduce false positive candidate terms. Perturbing documents as described will remove all false positives since the change in relevance score will be 0 when using reductive perturbation. For the same reason, we do not include \textsc{RM3-10}, \textsc{RM3-20} and \textsc{EMB}. Instead we consider 4 DESM variants:  \textsc{DESM-0.9}, \textsc{DESM-0.7}, \textsc{DESM-0.5} and \textsc{DESM-0.3}. The decrease in $\gamma$ is directly related to the certainty of false positives. It is harder to determine accuracy for \textsc{DESM-0.3} than for \textsc{DESM-0.9} since terms outside of $\mathcal{G}_q$ may also cause high semantic match.



%\subsection{Fidelity}

%To measure the local fidelity of the explanations we use two separate metrics. First we use spearman's coefficient as a measure of rank correlation. If $T_q$ is an accurate explanation then the correlation between the top k produced by $\mathcal{R}$ using q and $R$ using $T_q$ should be highly correlated. However this may not still accurately capture how $\mathcal{R}$ estimates the relevance of a document for a given query. To further test the fidelity of the explanation we measure the recall of $T_q$ given the query expansions used by $\mathcal{R}$ which is a retrieval model utilizing query expansions through pseudo relevance feedback. 

%\subsubsection{Objective - Rank Correlation}

%\subsubsection{True fidelity check with query expansion based RMs}

%Let $\mathcal{R}$ be a retrieval model that expands $q$ with a set of terms $\mathcal{T}_{q}$ before using $R$ to rank the retrieved documents. $\mathcal{T}_{q}$ can be determined in several ways. We experiment with the following methods: pseudo relevance feedback, word embeddings and topic models.  

%We measure fidelity as $f_q(R, \mathcal{R})@k = \frac{|T_q \cap \mathcal{T}_{q}|}{ | \mathcal{T}_{q} |}$

%\subsubsection{Human Fidelity Check for NNs}

%To measure fidelity to deep neural network rankers we propose using a human evaluation setup. Each participant is presented with the explanation from 3 different rankers for a given query. The user has to map the the ranking to the ranker based purely on a short description of the ranker and the explanation. To further control the setup we can use queries that result in nearly the same ranking for all rankers.



%\subsection{Utility}

%Utility of an explanation is measured in accordance with a downstream task. We select two such tasks: (i) select the model that will generalize better and (ii) predict the behavior of the ranker.

%\subsubsection{Generalization}

%Select 4 rankers that have similar training and validation set performance but vary considerably in test set performance. Show explanations from examples in the validation set. The user needs to pick the ranker which has best test set performance based on the explanations.

%\subsubsection{Predict behavior}

%Show the participant a ranking and explanation for a given $\mathcal{R}$ and query. Now show him/her a similar query and a small set of documents. Ask the participant to rank these documents according to what $\mathcal{R}$ would do. You can evaluate this by measuring user accuracy in this task.





